CaPa: Carve-n-Paint Synthesis for Efficient 4K Textured Mesh Generation

The synthesis of high-quality 3D assets from textual or visual inputs has become a central objective in modern generative modeling. Despite the proliferation of 3D generation algorithms, they frequently grapple with challenges such as multi-view inconsistency, slow generation times, low fidelity, and surface reconstruction problems. While some studies have addressed some of these issues, a comprehensive solution remains elusive. In this paper, we introduce \textbf{CaPa}, a carve-and-paint framework that generates high-fidelity 3D assets efficiently. CaPa employs a two-stage process, decoupling geometry generation from texture synthesis. Initially, a 3D latent diffusion model generates geometry guided by multi-view inputs, ensuring structural consistency across perspectives. Subsequently, leveraging a novel, model-agnostic Spatially Decoupled Attention, the framework synthesizes high-resolution textures (up to 4K) for a given geometry. Furthermore, we propose a 3D-aware occlusion inpainting algorithm that fills untextured regions, resulting in cohesive results across the entire model. This pipeline generates high-quality 3D assets in less than 30 seconds, providing ready-to-use outputs for commercial applications. Experimental results demonstrate that CaPa excels in both texture fidelity and geometric stability, establishing a new standard for practical, scalable 3D asset generation.

==> 01_intro_past.tex <==
\section{Introduction}
\label{sec:intro}
3D asset generation has become a critical technology in industries such as gaming, film, and virtual reality (VR), where the demand for high-quality, scalable 3D content continues to rise. Despite recent advancements in this field, existing methods still face significant challenges that limit their practicality. 
Lifting 2D generative models using a Score Distillation Sampling (SDS) \cite{poole2023dreamfusion, 23sjc} has laid foundational work, but they induce several limitations: the Janus problem—a common failure mode where textures on different sides of the object appear, meshing issues, and long generation times. 

The crux of the problem largely lies in how SDS-based methods rely on indirect 3D information distilled from 2D diffusion models, which sacrifices both quality and efficiency.
Aware of this problem, recent efforts in multi-view diffusion \cite{shi2024mvdream, wang2023imagedream} have addressed some of these limitations by designing models to predict multi-views from image or text inputs. % and lift them to 3D. 
Although this approach mitigates issues like the Janus problem, the other problems remain unresolved.

Beyond these multi-view inconsistencies, another critical limitation is the significant quality degradation when converting generated 3D assets into mesh form. 
Existing 3D asset generation methods predominantly attempt to produce both geometry and texture in a single unified process. 
However, these methods commonly utilize representations such as NeRF~\cite{mildenhall2020nerf} or Gaussian Splatting~\cite{kerbl3Dgaussians}, which are well-suited for neural rendering but inherently unsuitable for mesh-based applications~\cite{guedon24sugar,Huang242dgs,Yu2024GOF}. 
These representations often yield surfaces difficult to translate into high-quality, clean meshes, resulting in artifacts and quality degradation when the output is converted to a mesh.
% This issue arises due to two primary factors: 3D representations like NeRF \cite{mildenhall2020nerf} and Gaussian Splatting \cite{kerbl3Dgaussians}, while useful for neural rendering, are not optimized for surface reconstruction.
% It results in notable quality loss during the meshing process. 
% Additionally, most multi-view diffusion models are restricted to low resolution (typically, 256), inherently limiting the fidelity of the generated assets. 
% To circumvent the problem, some studies \cite{tang2024dreamgaussian, sun2024dreamcraftd} present a post-meshing refinement stage, re-optimizing the mesh with SDS loss to partially recover quality. This additional step, however, increases computational cost and complicates the workflow, reducing the practicality of these assets for real-world applications.

To address these limitations, we introduce \textbf{CaPa}, a two-stage \textit{Carve-n-Paint} framework that decouples geometry generation and texture synthesis, enhancing flexibility and performance at each stage.
This modular approach allows each component to be independently optimized, ensuring fast, robust, and high-fidelity results.

In the geometry generation stage, CaPa employs a 3D latent diffusion model that uses an occupancy field as its underlying representation, producing smoother and cleaner geometry that is easily mesh-compatible. 
Through this process, CaPa leverages multi-view images from the input view as guidance, enabling more precise geometry synthesis and ensuring better alignment with the texture synthesis stage.
The output of the stage is a high-quality mesh, which serves as a stable foundation for texture synthesis.
% In the geometry generation stage, CaPa employs a 3D latent diffusion model that predicts an occupancy field by denoising from a shape latent representation. Through this process, CaPa leverages multi-view images from the input view as guidance, enabling more precise geometry synthesis and ensuring better alignment with the texture synthesis stage.
% Unlike the recent Large Reconstruction Model (LRM) ~\cite{hong2024lrm} using NeRF, this occupancy-based representation is directly suitable for mesh conversion, such as marching cubes, enabling smoother, higher-quality surface extraction and minimizing quality loss during the meshing process.

% For texture synthesis, we first render the generated 3D mesh from four orthogonal views, guiding a 2D diffusion model to create the corresponding images. 
% At the core of this stage is Spatially Decoupled Cross Attention, a model-agnostic approach that generates seamless, Janus-free outputs. %seamless, Janus-free 4K textures. 
% Unlike MVDiffusion, which requires structural changes to the U-Net architecture and retraining, our method uses guidance from multi-view images by applying each to its designated spatial region during texture generation. 
% This allows Spatially Decoupled Cross Attention to work directly with large models like SDXL without modifying their architecture. 
% Additionally, while MVDiffusion lacks compatibility with pre-trained modules like ControlNet, our approach can leverage ControlNet~\cite{zhang23controlnet} trained for SDXL~\cite{podell2024sdxl}, enabling accurate, geometry-aligned textures. 
% This flexibility and efficiency make CaPa both highly adaptable and capable of delivering consistent, high-resolution textures.
For texture synthesis, we first render the generated 3D mesh from four orthogonal views, guiding a 2D diffusion model to create the corresponding high-fidelity images.
At the core of this stage is Spatially Decoupled Cross Attention, a model-agnostic method designed to ensure seamless, Janus-free textures.
This approach isolates and amplifies view-specific features within a unified diffusion process. 
Unlike MVDiffusion, which splits feature channels and requires custom cross-view attention layers, our method replicates channels for each view, allowing each spatial region to be processed independently in the unmodified U-Net architecture.
This design enables integration with large pre-trained models like SDXL~\cite{podell2024sdxl} without additional training, allowing us to leverage geometry-aware modules such as ControlNet~\cite{zhang23controlnet} for accurate, geometry-aligned textures.
Such flexibility ensures CaPa can generate high-resolution (4K) textures, achieving both versatile and highly effective for generating visually cohesive 3D assets.

Finally, to address untextured occluded regions left after back-projecting multi-view images onto the 3D mesh, we propose a novel 3D-aware occlusion inpainting algorithm. 
This algorithm generates a specialized UV map that captures mesh surface locality, facilitating efficient inpainting using 2D diffusion. 
Unlike standard UV-space inpainting methods~\cite{zeng24paint3d, siddiqui2024assetgen}, our 3D-aware approach preserves surface locality and minimizes seams in occluded regions.
% This method maintains high texture quality and consistency across the entire model by seamlessly filling occluded regions, avoiding visible seams.

Our extensive experiments demonstrate that our framework, CaPa, significantly outperforms existing methods in texture quality and geometric stability. It achieves high-resolution results (up to 4K) without the computational overhead typically associated with SDS-based techniques.

The core contributions of this work are summarized as:
\begin{itemize}
    \item \textbf{Mesh-Optimized 3D Generation Pipeline}: Separating geometry and texture generation, enabling effective meshing and enhancing the practicality of 3D asset generation.
    \item \textbf{Spatially Decoupled Cross Attention}: A model-agnostic, training-free solution to generate 4K textures without additional training, super-resolution, and janus problem. 
    \item \textbf{3D-aware Fast Occlusion Inpainting}: A robust inpainting solution for handling occluded regions in 3D textures, reducing visible seams, and preserving texture fidelity.
    \item \textbf{State-of-the-art Results}: CaPa achieves significantly higher texture and geometry fidelity, marking a major step forward in practical 3D asset generation.
\end{itemize}
% Another critical limitation in existing 3D generation methods is the inconsistency in view synthesis when using multi-view geometry extraction techniques. While pioneering works such as [c1, c2] have enabled impressive monocular geometry extraction, their multi-view counterparts, like Wonder3D, Direct2.5D, and Unique3D, often fall short in terms of geometric fidelity and texture consistency. These methods either rely too heavily on predicted normal maps or suffer from limited texture resolution, as seen in sparse NeRF-based approaches. Consequently, despite the efficient pipelines of these methods, the resulting assets frequently lack fine details and exhibit geometric instability or misaligned textures across views.

% Another critical limitation in existing 3D generation methods, particularly in approaches like Wonder3D and Unique3D, is the lack of view consistency when extracting geometric information for 3D asset generation. While optimization-based methods are less affected by this issue, view consistency becomes a critical challenge in methods that rely on sparse views (e.g., 4 or 6 views) for mesh optimization or NeRF reconstruction. In these approaches, without the accurate guidance of additional geometric information like normals, the quality of the generated assets significantly deteriorates. Furthermore, the inconsistency between views exacerbates these issues, leading to poor geometric fidelity and misaligned textures across different perspectives.

% To address these limitations, we propose a novel two-stage 3D generation framework, R3D2, which separates the process into geometry generation and texture synthesis. This modular approach allows us to leverage 3D-native networks for shape generation while utilizing 2D diffusion models to enhance texture fidelity. By separating shape and texture generation, our framework ensures that each component can be specialized and optimized independently, which leads to more robust results. Unlike the recently proposed Large Reconstruction Model (LRM), which employs 3D diffusion models for both geometry and texture, we leverage the 3D diffusion model exclusively for geometry generation, ensuring that texture synthesis remains flexible. 

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

